Redacting Transactions from Execute-Order-Validate Blockchains

As user privacy gains popularity and attention, and starts to shape relations between users and service providers, blockchain based solutions thrive for ways to relax immutability without sacrificing consistency. This work answers that need and presents the first design for a redactable execute-order-validate blockchain, that grants users with the \emph{right to be forgotten}. The design is easy to adopt, as we exemplify by implementing it on top of Hyperledger Fabric. It modifies the block structure and extracts user data from the hash-chain without loosening any correctness or liveness criteria. We evaluate our design and show that it provides compliance with only a minimal performance overhead, making it a feasible add-on to any execute-order-validate blockchain system.

==> Model.tex <==
\section{Model}
\Gal{should this be a subsection of the design section?}
In this section we provide a description of the model under which our design provides redaction ability. We refer to communication, failures, trust, and cryptographic assumptions. Further on, we formalize the problem statement.

% (Agnostic to the) Communication model
Our design, similar to \hlf~ is agnostic to the communication


% Failure model
Our solution does not compromise the resilience of any existing system it is applied on, namely, the design tolerates Byzantine failures. We later on show how such failures are contained. \Yacov{I don't understand how byzantine failures are related here,  why mentioning them? Also, this is not relevant to the model. The model is about who are the parties in the system, what kind of actors are they - honest, honest but curious, malicious, etc. and also what computational assumptions do we assume - CRH, signature un-forgability, etc.}


% Clients / trust?
\Yacov{I'm not sure why the following sentence is relevant to the model. This should be in introduction or in the design}
The addition of the redaction mechanism applies to multi-channel systems, as will be exemplified via \hlf. It does not require any additional trust, only updates to configuration and endorsement policy. 

% Crypto assumptions
% Collision free hash function
Our scheme relies on the collision-freedom property of the hash functions in use. Collision resistance means that the probability that two inputs (henceforth preimages to a function have the same output is negligible). This property will later allows determining matches between preimages and hashes with high confidence. Moreover, we use one-way hash functions, i.e., functions that are virtually irreversible: there does not exist an efficient way to retrieve the input to a function given its output. 


Similarly to any design relying on \Yacov{Let's formally define what is a cryptographic hash function and explain its 2 properties (one-wayness and collision resistance)} collision-free irreversible hash functions, ours also assumes that an adversarial input to a hash function which has the same output as a correct input cannot be calculated efficiently. 

% Formalize problem
We can now formalize the redaction problem for permissioned blockchains. Our requirements are as follows: \begin{enumerate}
	\item Successful redaction results in the deletion the user from the blockchain. Note that redaction does not revert the effect of the redacted transaction.
	\item Nodes joining the system will not be able to observe the contents of redacted transactions on the blockchain, had they received it from a majority of correct nodes.  \Yacov{Why is the majority important here?}\Gal{because if the majority is malicious, a newcomer may be convinced the world where the redacted transactions are present is the correct world state}
\end{enumerate}

